High-Performance Partial Spectrum Computation for Symmetric eigenvalue problems and the SVD

Current dense symmetric eigenvalue (EIG) and singular value decomposition (SVD) implementations may suffer from the lack of concurrency during the tridiagonal and bidiagonal reductions, respectively. This performance bottleneck is typical for the two-sided transformations due to the Level-2 BLAS memory-bound calls. Therefore, the current state-of-the-art EIG and SVD implementations may achieve only a small fraction of the system's sustained peak performance. The QR-based Dynamically Weighted Halley (QDWH) algorithm may be used as a pre-processing step toward the EIG and SVD solvers, while mitigating the aforementioned bottleneck. QDWH-EIG and QDWH-SVD expose more parallelism, while relying on compute-bound matrix operations. Both run closer to the sustained peak performance of the system, but at the expense of performing more FLOPS than the standard EIG and SVD algorithms. In this paper, we introduce a new QDWH-based solver for computing the partial spectrum for EIG (QDWHpartial-EIG) and SVD (QDWHpartial-SVD) problems. By optimizing the rational function underlying the algorithms only in the desired part of the spectrum, QDWHpartial-EIG and QDWHpartial-SVD algorithms efficiently compute a fraction (say 1-20%) of the corresponding spectrum. We develop high-performance implementations of QDWHpartial-EIG and QDWHpartial-SVD on distributed-memory anymore systems and demonstrate their numerical robustness. Experimental results using up to 36K MPI processes show performance speedups for QDWHpartial-SVD up to 6X and 2X against PDGESVD from ScaLAPACK and KSVD, respectively. QDWHpartial-EIG outperforms PDSYEVD from ScaLAPACK up to 3.5X but remains slower compared to ELPA. QDWHpartial-EIG achieves, however, a better occupancy of the underlying hardware by extracting higher sustained peak performance than ELPA, which is critical moving forward with accelerator-based supercomputers.

==> zolopd.tex <==
%!TEX root = qdwhpartial.tex
%=============================
As derived by Zolotarev, the type $(2r+1,2r)$ Zolotarev function 
for an integer $r\geq 1$
(the best rational approximant 
to the sign function) on $[-1,-\ell]\cup [l,\ell]$ is 
\begin{equation}
Z_{2r+1}(x;\ell) = Mx\Pi _{j=1}^{r} \frac{x^{2} + c_{2j}}{ x^{2} + c_{2j-1}},
\label{equ:zolo-sol}
\end{equation}
where $M > 0$ and satisfies the following:
$$ 1 - Z_{2r+1} (1;\ell) = -(1 - Z_{2r+1}(l;\ell)).$$
The scalars $c_{1}, c_{2}, \dots, c_{2r}$ can be computed using the Jacobi 
elliptic functions $sn(u;\ell')$, $cn(u;\ell')$. 
Evaluating $Z_{2r+1}(x;\ell)$ at a matrix argument $X$ to 
obtain $UZ_{2r+1}(\Sigma;\ell)V^*$ where $X=U\Sigma V^*$ is the SVD can be done by
\[Z_{2r+1}(X;\ell) = MX\Pi_{j=1}^{r} (X^*X + c_{2j}I) (X^*X + c_{2j-1}I)^{-1}.\]
QDWH represents Zolotarev functions of type $(3,2)$. 
We rewrite this in partial fraction form, to improve the degree of parallelism: 
we can find $a_j\in\mathbb{R}$ such that 
\begin{equation}
Z_{2r+1}(X;\ell) = M(X + \Sigma_{j=1}^{r} a_{j} X (X^*X + c_{2j-1}I)^{-1}).
\label{equ:zolo-sol-parfun}
\end{equation}
Similar to QDWH which represents Zolotarev functions of type $(3,2)$, 
$Z_{2r+1}(X;\ell)$ in Equation~\eqref{equ:zolo-sol-parfun} can be computed stably as
\begin{equation}
\begin{aligned}
\begin{bmatrix}
X \\
\sqrt{c_{2j-1}} I
\end{bmatrix} &=
\begin{bmatrix}
Q_{j1} \\
Q_{j2} 
\end{bmatrix}
R_{j},\\
%R(X) = 
Z_{2r+1}(X;\ell)&=X + \Sigma_{j=1}^{r} \frac{a_{j}}{\sqrt{c_{2j-1}}}Q_{j1}Q_{j2}^{*}.
\end{aligned}
\label{equ:rat-fun-qr}
\end{equation}
%Equation~\ref{equ:rat-fun-qr}
This represents a number of \emph{r} embarrassingly parallel $QR$ factorizations and matrix-matrix multiplications 
$Q_{j1} Q_{j2}^{*}$. The upshot of ZOLO-PD is that by taking $r=8$, we obtain 
$\|Z_{2r+1}(Z_{2r+1}(A;\ell_0);\ell_1)-U_p\|\leq 10^{-15}$  for any $A$ with $\kappa_2(A)\leq 10^{12}$, 
implying that convergence is attained in just two steps. 

The $QR$ iterations in~\eqref{equ:rat-fun-qr} can be reformulated
as Cholesky-based iterations with a lower arithmetic cost, as in~\eqref{practical-polar-chol}, 
once $X_k$ is well-conditioned. 
%And because of the ZOLO-PD seventeen convergence rate, 
This condition is already satisfied at the second iteration even for ill-conditioned matrices.

The ZOLO-PD algorithm~\cite{Yuji2016} can be seen as a generalization of QDWH 
into a series of independent QDWH subproblems with only two iterations per 
subproblem, instead of the original six iterations, as mentioned in Section~\ref{subsec:qdwhpd}.
We have already demonstrated the performance superiority of ZOLO-PD over QDWH in the context of strong scaling
mode of operation~\cite{ltaief2019}. For the subsequent sections of the paper, we
focus on QDWH without loss of generality.

The next section highlights the application of QDWH as a pre-processing step
toward computing the symmetric eigendecomposition and SVD.

